Towards Unified Representation of Multi-Modal Pre-training for 3D Understanding via Differentiable Rendering

State-of-the-art 3D models, which excel in recognition tasks, typically depend on large-scale datasets and well-defined category sets. Recent advances in multi-modal pre-training have demonstrated potential in learning 3D representations by aligning features from 3D shapes with their 2D RGB or depth counterparts. However, these existing frameworks often rely solely on either RGB or depth images, limiting their effectiveness in harnessing a comprehensive range of multi-modal data for 3D applications. To tackle this challenge, we present DR-Point, a tri-modal pre-training framework that learns a unified representation of RGB images, depth images, and 3D point clouds by pre-training with object triplets garnered from each modality. To address the scarcity of such triplets, DR-Point employs differentiable rendering to obtain various depth images. This approach not only augments the supply of depth images but also enhances the accuracy of reconstructed point clouds, thereby promoting the representative learning of the Transformer backbone. Subsequently, using a limited number of synthetically generated triplets, DR-Point effectively learns a 3D representation space that aligns seamlessly with the RGB-Depth image space. Our extensive experiments demonstrate that DR-Point outperforms existing self-supervised learning methods in a wide range of downstream tasks, including 3D object classification, part segmentation, point cloud completion, semantic segmentation, and detection. Additionally, our ablation studies validate the effectiveness of DR-Point in enhancing point cloud understanding.

==> Tables/MVP.tex <==

\begin{table*}[t]
\caption{\textbf{The comparison of DR-Point fine-tuned on MVP dataset with other train-from-scratch networks regarding CD-${\ell}_1$ {$\times 10^3$}, CD-${\ell}_2$ {$\times 10^3$} as well as average F-Score@1{$\%$}.}}
\resizebox{\textwidth}{!}{%
\begin{tabular}{c|cccccccccccccccc|c}
\toprule[1.5pt]
\rowcolor[HTML]{FFFFFF} 
Methods &
  Airplane &
  Bed &
  Bench &
  Bookshelf &
  Bus &
  Cabinet &
  Car &
  Chair &
  Guitar &
  Lamp &
  Motorbike &
  Pistol &
  Skateboard &
  Sofa &
  Table &
  Watercraft &
  Avg. \\ \midrule[1pt]
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF}F-Score/ &
  \cellcolor[HTML]{FFFFFF}F-Score/ &
  \cellcolor[HTML]{FFFFFF}F-Score/ &
  \cellcolor[HTML]{FFFFFF}F-Score/ &
  \cellcolor[HTML]{FFFFFF}F-Score/ &
  \cellcolor[HTML]{FFFFFF}F-Score/ &
  \cellcolor[HTML]{FFFFFF}F-Score/ &
  \cellcolor[HTML]{FFFFFF}F-Score/ &
  \cellcolor[HTML]{FFFFFF}F-Score/ &
  F-Score/ &
  F-Score/ &
  F-Score/ &
  F-Score/ &
  F-Score/ &
  F-Score/ &
  F-Score/ &
  F-Score/ \\
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF}CD-$\ell_1$/ &
  \cellcolor[HTML]{FFFFFF}CD-$\ell_1$/ &
  \cellcolor[HTML]{FFFFFF}CD-$\ell_1$/ &
  \cellcolor[HTML]{FFFFFF}CD-$\ell_1$/ &
  \cellcolor[HTML]{FFFFFF}CD-$\ell_1$/ &
  \cellcolor[HTML]{FFFFFF}CD-$\ell_1$/ &
  \cellcolor[HTML]{FFFFFF}CD-$\ell_1$/ &
  \cellcolor[HTML]{FFFFFF}CD-$\ell_1$/ &
  \cellcolor[HTML]{FFFFFF}CD-$\ell_1$/ &
  CD-$\ell_1$/ &
  CD-$\ell_1$/ &
  CD-$\ell_1$/ &
  CD-$\ell_1$/ &
  CD-$\ell_1$/ &
  CD-$\ell_1$/ &
  CD-$\ell_1$/ &
  CD-$\ell_1$/ \\
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF}CD-$\ell_2$ &
  \cellcolor[HTML]{FFFFFF}CD-$\ell_2$ &
  \cellcolor[HTML]{FFFFFF}CD-$\ell_2$ &
  \cellcolor[HTML]{FFFFFF}CD-$\ell_2$ &
  \cellcolor[HTML]{FFFFFF}CD-$\ell_2$ &
  \cellcolor[HTML]{FFFFFF}CD-$\ell_2$ &
  \cellcolor[HTML]{FFFFFF}CD-$\ell_2$ &
  \cellcolor[HTML]{FFFFFF}CD-$\ell_2$ &
  \cellcolor[HTML]{FFFFFF}CD-$\ell_2$ &
  CD-$\ell_2$ &
  CD-$\ell_2$ &
  CD-$\ell_2$ &
  CD-$\ell_2$ &
  CD-$\ell_2$ &
  CD-$\ell_2$ &
  CD-$\ell_2$ &
  CD-$\ell_2$ \\ \midrule[1pt]
\rowcolor[HTML]{EFEFEF} 
 &
  0.857 &
  0.438 &
  0.674 &
  0.461 &
  0.673 &
  0.486 &
  0.533 &
  0.517 &
  0.886 &
  0.593 &
  0.626 &
  0.749 &
  0.822 &
  0.473 &
  0.587 &
  0.632 &
  0.605 \\
\rowcolor[HTML]{EFEFEF} 
ASFMNet~\cite{xia2021asfm} &
  6.530 &
  16.810 &
  10.496 &
  14.105 &
  9.240 &
  12.285 &
  10.861 &
  13.799 &
  5.571 &
  14.510 &
  9.868 &
  8.456 &
  7.263 &
  13.210 &
  12.687 &
  11.351 &
  11.484 \\
\rowcolor[HTML]{EFEFEF} 
 &
  0.234 &
  1.567 &
  0.617 &
  1.087 &
  0.345 &
  0.597 &
  0.405 &
  0.879 &
  0.109 &
  1.336 &
  0.328 &
  0.354 &
  0.357 &
  0.685 &
  0.972 &
  0.669 &
  0.691 \\
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF}0.825 &
  \cellcolor[HTML]{FFFFFF}0.467 &
  \cellcolor[HTML]{FFFFFF}0.645 &
  \cellcolor[HTML]{FFFFFF}0.504 &
  \cellcolor[HTML]{FFFFFF}0.679 &
  \cellcolor[HTML]{FFFFFF}0.550 &
  \cellcolor[HTML]{FFFFFF}0.613 &
  \cellcolor[HTML]{FFFFFF}0.501 &
  \cellcolor[HTML]{FFFFFF}0.815 &
  0.536 &
  0.668 &
  0.740 &
  0.778 &
  0.497 &
  0.579 &
  0.635 &
  0.609 \\
\cellcolor[HTML]{FFFFFF}GRNet~\cite{xie2020grnet} &
  \cellcolor[HTML]{FFFFFF}7.134 &
  \cellcolor[HTML]{FFFFFF}16.535 &
  \cellcolor[HTML]{FFFFFF}11.252 &
  \cellcolor[HTML]{FFFFFF}14.026 &
  \cellcolor[HTML]{FFFFFF}9.769 &
  \cellcolor[HTML]{FFFFFF}12.202 &
  \cellcolor[HTML]{FFFFFF}10.466 &
  \cellcolor[HTML]{FFFFFF}14.705 &
  \cellcolor[HTML]{FFFFFF}6.684 &
  15.735 &
  9.492 &
  8.396 &
  8.719 &
  13.531 &
  13.149 &
  10.833 &
  11.817 \\
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF}0.336 &
  \cellcolor[HTML]{FFFFFF}1.302 &
  \cellcolor[HTML]{FFFFFF}0.610 &
  \cellcolor[HTML]{FFFFFF}0.890 &
  \cellcolor[HTML]{FFFFFF}0.374 &
  \cellcolor[HTML]{FFFFFF}0.558 &
  \cellcolor[HTML]{FFFFFF}0.366 &
  \cellcolor[HTML]{FFFFFF}0.915 &
  \cellcolor[HTML]{FFFFFF}0.163 &
  1.431 &
  0.302 &
  0.276 &
  0.701 &
  0.670 &
  0.902 &
  0.530 &
  0.679 \\
\rowcolor[HTML]{EFEFEF} 
 &
  0.891 &
  0.527 &
  0.704 &
  0.626 &
  0.718 &
  0.674 &
  0.734 &
  0.656 &
  0.644 &
  0.665 &
  0.623 &
  0.594 &
  0.700 &
  0.639 &
  0.726 &
  0.732 &
  0.696 \\
\rowcolor[HTML]{EFEFEF} 
CRN~\cite{wang2021cascaded} &
  5.495 &
  18.480 &
  11.440 &
  12.509 &
  9.507 &
  10.064 &
  8.641 &
  11.367 &
  12.745 &
  12.111 &
  11.346 &
  16.773 &
  11.478 &
  10.825 &
  10.389 &
  9.186 &
  10.579 \\
\rowcolor[HTML]{EFEFEF} 
 &
  0.190 &
  2.139 &
  0.853 &
  1.018 &
  0.405 &
  0.404 &
  0.264 &
  0.625 &
  0.899 &
  0.954 &
  0.525 &
  1.974 &
  0.758 &
  0.488 &
  0.724 &
  0.436 &
  0.651 \\
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF}0.747 &
  \cellcolor[HTML]{FFFFFF}0.327 &
  \cellcolor[HTML]{FFFFFF}0.595 &
  \cellcolor[HTML]{FFFFFF}0.347 &
  \cellcolor[HTML]{FFFFFF}0.618 &
  \cellcolor[HTML]{FFFFFF}0.420 &
  \cellcolor[HTML]{FFFFFF}0.511 &
  \cellcolor[HTML]{FFFFFF}0.342 &
  \cellcolor[HTML]{FFFFFF}0.812 &
  0.336 &
  0.532 &
  0.638 &
  0.754 &
  0.364 &
  0.501 &
  0.485 &
  0.492 \\
\cellcolor[HTML]{FFFFFF}TopNet~\cite{tchapmi2019topnet} &
  \cellcolor[HTML]{FFFFFF}7.979 &
  \cellcolor[HTML]{FFFFFF}16.529 &
  \cellcolor[HTML]{FFFFFF}11.043 &
  \cellcolor[HTML]{FFFFFF}14.796 &
  \cellcolor[HTML]{FFFFFF}9.797 &
  \cellcolor[HTML]{FFFFFF}12.617 &
  \cellcolor[HTML]{FFFFFF}11.053 &
  \cellcolor[HTML]{FFFFFF}14.895 &
  \cellcolor[HTML]{FFFFFF}6.760 &
  16.765 &
  10.868 &
  9.492 &
  7.875 &
  13.988 &
  12.929 &
  12.537 &
  12.357 \\
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF}0.286 &
  \cellcolor[HTML]{FFFFFF}1.023 &
  \cellcolor[HTML]{FFFFFF}0.493 &
  \cellcolor[HTML]{FFFFFF}0.779 &
  \cellcolor[HTML]{FFFFFF}0.316 &
  \cellcolor[HTML]{FFFFFF}0.508 &
  \cellcolor[HTML]{FFFFFF}0.370 &
  \cellcolor[HTML]{FFFFFF}0.741 &
  \cellcolor[HTML]{FFFFFF}0.153 &
  1.189 &
  0.372 &
  0.321 &
  0.218 &
  0.599 &
  0.674 &
  0.637 &
  0.584 \\
\rowcolor[HTML]{EFEFEF} 
 &
  0.739 &
  0.309 &
  0.604 &
  0.407 &
  0.705 &
  0.496 &
  0.572 &
  0.334 &
  0.848 &
  0.320 &
  0.511 &
  0.706 &
  0.782 &
  0.392 &
  0.518 &
  0.515 &
  0.516 \\
\rowcolor[HTML]{EFEFEF} 
FoldingNet~\cite{yang2018foldingnet} &
  8.144 &
  15.940 &
  10.948 &
  12.359 &
  8.650 &
  11.246 &
  10.180 &
  14.668 &
  6.255 &
  17.878 &
  10.928 &
  8.576 &
  9.418 &
  13.041 &
  11.966 &
  11.923 &
  11.881 \\
\rowcolor[HTML]{EFEFEF} 
 &
  0.339 &
  1.022 &
  0.636 &
  0.561 &
  0.255 &
  0.412 &
  0.314 &
  0.754 &
  0.120 &
  1.536 &
  0.358 &
  0.268 &
  1.267 &
  0.570 &
  0.572 &
  0.563 &
  0.615 \\
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF}0.785 &
  \cellcolor[HTML]{FFFFFF}0.334 &
  \cellcolor[HTML]{FFFFFF}0.559 &
  \cellcolor[HTML]{FFFFFF}0.461 &
  \cellcolor[HTML]{FFFFFF}0.746 &
  \cellcolor[HTML]{FFFFFF}0.570 &
  \cellcolor[HTML]{FFFFFF}0.641 &
  \cellcolor[HTML]{FFFFFF}0.387 &
  \cellcolor[HTML]{FFFFFF}0.879 &
  0.357 &
  0.607 &
  0.705 &
  0.816 &
  0.453 &
  0.538 &
  0.529 &
  0.559 \\
\cellcolor[HTML]{FFFFFF}PCN~\cite{yuan2018pcn} &
  \cellcolor[HTML]{FFFFFF}7.951 &
  \cellcolor[HTML]{FFFFFF}20.999 &
  \cellcolor[HTML]{FFFFFF}14.019 &
  \cellcolor[HTML]{FFFFFF}15.830 &
  \cellcolor[HTML]{FFFFFF}8.920 &
  \cellcolor[HTML]{FFFFFF}11.997 &
  \cellcolor[HTML]{FFFFFF}10.358 &
  \cellcolor[HTML]{FFFFFF}17.882 &
  \cellcolor[HTML]{FFFFFF}5.643 &
  22.093 &
  10.963 &
  9.885 &
  7.676 &
  14.694 &
  14.841 &
  13.921 &
  13.598 \\
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF}0.374 &
  \cellcolor[HTML]{FFFFFF}1.938 &
  \cellcolor[HTML]{FFFFFF}0.987 &
  \cellcolor[HTML]{FFFFFF}1.178 &
  \cellcolor[HTML]{FFFFFF}0.323 &
  \cellcolor[HTML]{FFFFFF}0.543 &
  \cellcolor[HTML]{FFFFFF}0.373 &
  \cellcolor[HTML]{FFFFFF}1.240 &
  \cellcolor[HTML]{FFFFFF}0.120 &
  2.363 &
  0.431 &
  0.558 &
  0.347 &
  0.795 &
  1.119 &
  0.856 &
  0.902 \\
\rowcolor[HTML]{EFEFEF} 
 &
  0.843 &
  0.644 &
  0.804 &
  0.707 &
  0.814 &
  0.681 &
  0.726 &
  0.682 &
  0.779 &
  0.714 &
  0.784 &
  0.841 &
  0.900 &
  0.649 &
  0.759 &
  0.750 &
  0.740 \\
\rowcolor[HTML]{EFEFEF} 
ECG~\cite{pan2020ecg} &
  6.189 &
  11.956 &
  7.850 &
  9.870 &
  7.055 &
  9.635 &
  8.180 &
  10.168 &
  6.734 &
  10.711 &
  7.448 &
  6.552 &
  5.542 &
  10.002 &
  9.032 &
  8.450 &
  8.753 \\
\rowcolor[HTML]{EFEFEF} 
 &
  0.185 &
  0.859 &
  0.375 &
  0.520 &
  0.216 &
  0.385 &
  0.243 &
  0.522 &
  0.179 &
  0.881 &
  0.209 &
  0.235 &
  0.156 &
  0.429 &
  0.506 &
  0.394 &
  0.418 \\
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF}0.916 &
  \cellcolor[HTML]{FFFFFF}0.654 &
  \cellcolor[HTML]{FFFFFF}0.853 &
  \cellcolor[HTML]{FFFFFF}0.728 &
  \cellcolor[HTML]{FFFFFF}0.842 &
  \cellcolor[HTML]{FFFFFF}0.729 &
  \cellcolor[HTML]{FFFFFF}0.751 &
  \cellcolor[HTML]{FFFFFF}0.725 &
  \cellcolor[HTML]{FFFFFF}0.952 &
  0.737 &
  0.796 &
  0.868 &
  0.924 &
  0.717 &
  0.795 &
  0.791 &
  0.784 \\
\cellcolor[HTML]{FFFFFF}PoinTr~\cite{yu2021pointr} &
  \cellcolor[HTML]{FFFFFF}4.806 &
  \cellcolor[HTML]{FFFFFF}11.921 &
  \cellcolor[HTML]{FFFFFF}6.948 &
  \cellcolor[HTML]{FFFFFF}9.438 &
  \cellcolor[HTML]{FFFFFF}6.781 &
  \cellcolor[HTML]{FFFFFF}9.343 &
  \cellcolor[HTML]{FFFFFF}8.293 &
  \cellcolor[HTML]{FFFFFF}9.369 &
  \cellcolor[HTML]{FFFFFF}4.089 &
  9.465 &
  7.447 &
  6.176 &
  5.141 &
  9.490 &
  8.469 &
  7.533 &
  8.070 \\
\cellcolor[HTML]{FFFFFF} &
  \cellcolor[HTML]{FFFFFF}0.134 &
  \cellcolor[HTML]{FFFFFF}0.818 &
  \cellcolor[HTML]{FFFFFF}0.272 &
  \cellcolor[HTML]{FFFFFF}0.439 &
  \cellcolor[HTML]{FFFFFF}0.193 &
  \cellcolor[HTML]{FFFFFF}0.374 &
  \cellcolor[HTML]{FFFFFF}0.240 &
  \cellcolor[HTML]{FFFFFF}0.398 &
  \cellcolor[HTML]{FFFFFF}0.056 &
  0.615 &
  0.188 &
  0.185 &
  0.107 &
  0.381 &
  0.444 &
  0.267 &
  0.338 \\
\rowcolor[HTML]{EFEFEF} 
 &
  0.934 &
  0.709 &
  0.874 &
  0.787 &
  0.848 &
  0.763 &
  0.766 &
  0.762 &
  0.969 &
  0.782 &
  0.833 &
  0.893 &
  0.943 &
  0.742 &
  0.840 &
  0.797 &
  0.813 \\
\rowcolor[HTML]{EFEFEF} 
SnowflakeNet~\cite{xiang2021snowflakenet} &
  4.393 &
  10.750 &
  6.431 &
  8.383 &
  6.735 &
  9.056 &
  8.052 &
  8.772 &
  3.454 &
  9.159 &
  6.905 &
  5.722 &
  4.458 &
  9.035 &
  7.551 &
  7.404 &
  7.597 \\
\rowcolor[HTML]{EFEFEF} 
\textbf{} &
  0.113 &
  0.736 &
  0.264 &
  0.380 &
  0.206 &
  0.403 &
  0.238 &
  0.405 &
  0.042 &
  0.690 &
  0.167 &
  0.170 &
  0.121 &
  0.388 &
  0.391 &
  0.285 &
  0.338 \\ \midrule[1pt]
\cellcolor[HTML]{FFFFFF} & 
  \cellcolor[HTML]{FFFFFF}\textbf{0.946 } & 
  \cellcolor[HTML]{FFFFFF}\textbf{0.731 } & 
  \cellcolor[HTML]{FFFFFF}\textbf{0.891 } & 
  \cellcolor[HTML]{FFFFFF}\textbf{0.803 } &  
  \cellcolor[HTML]{FFFFFF}\textbf{0.837 } &  
  \cellcolor[HTML]{FFFFFF}\textbf{0.741 }  & 
  \cellcolor[HTML]{FFFFFF}\textbf{0.739  }  &
  \cellcolor[HTML]{FFFFFF}\textbf{0.789  } & 
  \cellcolor[HTML]{FFFFFF}\textbf{0.977  } & 
  \textbf{0.858 } &  	
  \textbf{0.858 } & 
  \textbf{0.899 } & 
  \textbf{0.943 } & 
  \textbf{0.745 } & 
  \textbf{0.844 } & 
  \textbf{0.829 } &
  \textbf{ 0.825 } \\
\cellcolor[HTML]{FFFFFF} \textbf{DR-Point} & 
  \cellcolor[HTML]{FFFFFF}\textbf{3.781 } & 
  \cellcolor[HTML]{FFFFFF}\textbf{8.811 } & 
  \cellcolor[HTML]{FFFFFF}\textbf{5.495 } & 
  \cellcolor[HTML]{FFFFFF}\textbf{7.441 } & 
  \cellcolor[HTML]{FFFFFF}\textbf{6.286 } & 
  \cellcolor[HTML]{FFFFFF}\textbf{8.385 } & 
  \cellcolor[HTML]{FFFFFF}\textbf{7.688 } & 
  \cellcolor[HTML]{FFFFFF}\textbf{7.198 } & 
  \cellcolor[HTML]{FFFFFF}\textbf{3.097 } & 
  \textbf{5.796 } & 
  \textbf{6.428 } & 
  \textbf{5.113 } & 
  \textbf{4.264 } & 
  \textbf{7.870 } & 
  \textbf{6.596 } & 
  \textbf{6.090 } & 
  \textbf{6.473 } \\
\cellcolor[HTML]{FFFFFF}\textbf{} & 
  \cellcolor[HTML]{FFFFFF}\textbf{0.068 } & 
  \cellcolor[HTML]{FFFFFF}\textbf{0.479 } & 
  \cellcolor[HTML]{FFFFFF}\textbf{0.171 } & 
  \cellcolor[HTML]{FFFFFF}\textbf{0.276 } & 
  \cellcolor[HTML]{FFFFFF}\textbf{0.170 } & 
  \cellcolor[HTML]{FFFFFF}\textbf{0.297 } & 
  \cellcolor[HTML]{FFFFFF}\textbf{0.215 } & 
  \cellcolor[HTML]{FFFFFF}\textbf{0.265 } & 
  \cellcolor[HTML]{FFFFFF}\textbf{0.036 } & 
  \textbf{0.234 } & 
  \textbf{0.141 } & 
  \textbf{0.124 } & 
  \textbf{0.122 } & 
  \textbf{0.284 } & 
  \textbf{0.268 } & 
  \textbf{0.195 } & 
  \textbf{0.219 } \\ \bottomrule[1.5pt]
\end{tabular}
}

\label{table:completion-MVP}
\end{table*}


==> Tables/PCN.tex <==

\begin{table*}[htbp]\scriptsize
\centering
% \tabcolsep=0.09cm
% \renewcommand{\arraystretch}{0.8}
\caption{\textbf{The comparison of DR-Point fine-tuned on PCN dataset and other train-from-scratch networks regarding CD-${\ell}_1$ {$\times 10^3$}, CD-${\ell}_2$ {$\times 10^3$} and the average F-Score@1{$\%$}.}}
\vspace{-0.3cm}
{
\begin{tabular}{c|ccccccccc}
\toprule[1.5pt]
\rowcolor[HTML]{FFFFFF} 
Methods          & Airplane & Cabinet & Car    & Chair  & Lamp   & Sofa   & Table  & Watercraft                                          & Avg.   \\ \midrule[1pt]
\rowcolor[HTML]{FFFFFF} 
 &
  F-Score/ &
  F-Score/ &
  F-Score/ &
  F-Score/ &
  F-Score/ &
  F-Score/ &
  F-Score/ &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}F-Score/} &
  F-Score/ \\
\rowcolor[HTML]{FFFFFF} 
 &
  CD-$\ell_1$/ &
  CD-$\ell_1$/ &
  CD-$\ell_1$/ &
  CD-$\ell_1$/ &
  CD-$\ell_1$/ &
  CD-$\ell_1$/ &
  CD-$\ell_1$/ &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}CD-$\ell_1$/} &
  CD-$\ell_1$/ \\
\rowcolor[HTML]{FFFFFF} 
 &
  CD-$\ell_2$ &
  CD-$\ell_2$ &
  CD-$\ell_2$ &
  CD-$\ell_2$ &
  CD-$\ell_2$ &
  CD-$\ell_2$ &
  CD-$\ell_2$ &
  \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}CD-$\ell_2$} &
  CD-$\ell_2$ \\ \midrule[1pt]
\rowcolor[HTML]{EFEFEF} 
                 & 0.738    & 0.330   & 0.409  & 0.399  & 0.496  & 0.331  & 0.411  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.556}  & 0.459  \\
\rowcolor[HTML]{EFEFEF} 
ASFMNet~\cite{xia2021asfm}          & 8.792    & 17.800  & 13.730 & 16.300 & 16.030 & 17.620 & 16.540 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}12.460} & 14.910 \\
\rowcolor[HTML]{EFEFEF} 
                 & 0.334    & 1.158   & 0.597  & 1.030  & 1.187  & 1.180  & 1.212  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.647}  & 0.918  \\
\rowcolor[HTML]{FFFFFF} 
                 & 0.711    & 0.447   & 0.507  & 0.483  & 0.609  & 0.415  & 0.556  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.603}  & 0.541  \\
\rowcolor[HTML]{FFFFFF} 
GRNet~\cite{xie2020grnet}           & 9.433    & 14.930  & 12.020 & 14.520 & 12.170 & 15.420 & 12.780 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}11.020} & 12.790 \\
\rowcolor[HTML]{FFFFFF} 
                 & 0.405    & 0.786   & 0.462  & 0.808  & 0.689  & 0.950  & 0.672  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.525}  & 0.662  \\
\rowcolor[HTML]{EFEFEF} 
                 & 0.804    & 0.439   & 0.486  & 0.505  & 0.533  & 0.409  & 0.606  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.607}  & 0.549  \\
\rowcolor[HTML]{EFEFEF} 
CRN~\cite{wang2021cascaded}             & 7.892    & 14.230  & 12.750 & 13.350 & 13.680 & 15.290 & 11.520 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}11.090} & 12.470 \\
\rowcolor[HTML]{EFEFEF} 
                 & 0.351    & 0.704   & 0.526  & 0.653  & 0.842  & 0.842  & 0.570  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.480}  & 0.628  \\
\rowcolor[HTML]{FFFFFF} 
                 & 0.760    & 0.321   & 0.496  & 0.342  & 0.345  & 0.313  & 0.504  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.461}  & 0.443  \\
\rowcolor[HTML]{FFFFFF} 
TopNet~\cite{tchapmi2019topnet}           & 7.785    & 14.940  & 11.640 & 15.450 & 14.040 & 15.260 & 12.300 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}12.320} & 12.970 \\
\rowcolor[HTML]{FFFFFF} 
                 & 0.240    & 0.712   & 0.404  & 0.856  & 0.710  & 0.771  & 0.595  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.504}  & 0.599  \\
\rowcolor[HTML]{EFEFEF} 
                 & 0.723    & 0.310   & 0.488  & 0.307  & 0.332  & 0.280  & 0.457  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.449}  & 0.418  \\
\rowcolor[HTML]{EFEFEF} 
FoldingNet~\cite{yang2018foldingnet}      & 8.283    & 14.240  & 11.100 & 14.590 & 13.990 & 14.630 & 12.800 & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}12.300} & 12.740 \\
\rowcolor[HTML]{EFEFEF} 
                 & 0.264    & 0.665   & 0.355  & 0.719  & 0.733  & 0.687  & 0.624  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.514}  & 0.570  \\
\rowcolor[HTML]{FFFFFF} 
                 & 0.831    & 0.508   & 0.649  & 0.506  & 0.522  & 0.433  & 0.621  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.644}  & 0.589  \\
\rowcolor[HTML]{FFFFFF} 
PCN~\cite{yuan2018pcn}              & 6.825    & 12.950  & 9.953  & 13.170 & 13.370 & 14.430 & 11.450 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}10.490} & 11.580 \\
\rowcolor[HTML]{FFFFFF} 
                 & 0.213    & 0.633   & 0.313  & 0.638  & 0.750  & 0.784  & 0.573  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.433}  & 0.542  \\
\rowcolor[HTML]{EFEFEF} 
                 & 0.870    & 0.605   & 0.675  & 0.635  & 0.698  & 0.502  & 0.730  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.759}  & 0.684  \\
\rowcolor[HTML]{EFEFEF} 
ECG~\cite{pan2020ecg}              & 6.069    & 11.150  & 8.986  & 10.700 & 10.080 & 12.780 & 9.114  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}8.171}  & 9.631  \\
\rowcolor[HTML]{EFEFEF} 
                 & 0.169    & 0.502   & 0.253  & 0.459  & 0.570  & 0.632  & 0.380  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.299}  & 0.408  \\
\rowcolor[HTML]{FFFFFF} 
                 & 0.834    & 0.522   & 0.585  & 0.556  & 0.648  & 0.475  & 0.668  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.689}  & 0.622  \\
\rowcolor[HTML]{FFFFFF} 
PoinTr~\cite{yu2021pointr}          & 6.553    & 12.710  & 10.540 & 11.750 & 10.430 & 13.400 & 10.430 & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}8.939}  & 10.600 \\
\rowcolor[HTML]{FFFFFF} 
                 & 0.184    & 0.634   & 0.357  & 0.522  & 0.515  & 0.761  & 0.618  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}0.290}  & 0.485  \\
\rowcolor[HTML]{EFEFEF} 
                 & 0.897    & 0.648   & 0.697  & 0.705  & 0.790  & 0.604  & 0.820  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.787}  & 0.743  \\
\rowcolor[HTML]{EFEFEF} 
SnowflakeNet~\cite{xiang2021snowflakenet}     & 5.262    & 10.370  & 8.847  & 9.103  & 7.717  & 10.710 & 7.663  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}7.221}  & 8.362  \\
\rowcolor[HTML]{EFEFEF} 
\textbf{}        & 0.131    & 0.439   & 0.246  & 0.343  & 0.343  & 0.493  & 0.294  & \multicolumn{1}{c|}{\cellcolor[HTML]{EFEFEF}0.196}  & 0.311  \\ \midrule[1pt]
\rowcolor[HTML]{FFFFFF} 
                 & \textbf{0.926}   & \textbf{0.645}  & \textbf{0.705}   & \textbf{0.744}   & \textbf{0.848}  & \textbf{0.635}  & \textbf{0.836} & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.831}}  & \textbf{0.771}  \\
\rowcolor[HTML]{FFFFFF} 
\textbf{DR-Point} & \textbf{4.390}    & \textbf{9.994}   & \textbf{8.479}  & \textbf{8.061}  & \textbf{5.976}  & \textbf{9.913}  & \textbf{6.799}  & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{6.215}}  & \textbf{7.478} \\
\rowcolor[HTML]{FFFFFF} 
\textbf{}        & \textbf{0.129}   & \textbf{0.428}   & \textbf{0.246}  & \textbf{0.301}  & \textbf{0.214}  & \textbf{0.470}  & \textbf{0.245}   & \multicolumn{1}{c|}{\cellcolor[HTML]{FFFFFF}\textbf{0.175}}  & \textbf{0.276} \\ \bottomrule[1.5pt]
\end{tabular}}

\label{table:completion-PCN}
\end{table*}
